Cortical Morphometry Analysis based on Worst Transportation Theory

Biomarkers play an important role in early detection and intervention in Alzheimer's disease (AD). However, obtaining effective biomarkers for AD is still a big challenge. In this work, we propose to use the worst transportation cost as a univariate biomarker to index cortical morphometry for tracking AD progression. The worst transportation (WT) aims to find the least economical way to transport one measure to the other, which contrasts to the optimal transportation (OT) that finds the most economical way between measures. To compute the WT cost, we generalize the Brenier theorem for the OT map to the WT map, and show that the WT map is the gradient of a concave function satisfying the Monge-Ampere equation. We also develop an efficient algorithm to compute the WT map based on computational geometry. We apply the algorithm to analyze cortical shape difference between dementia due to AD and normal aging individuals. The experimental results reveal the effectiveness of our proposed method which yields better statistical performance than other competiting methods including the OT.

==> Alexandrov.tex <==
\chapter{Spherical Optimal Transport}
\begin{figure}[t!]
    \centering
\begin{tabular}{c}
\includegraphics[height=0.45\textwidth]{figures/Alexandrov_Duality.pdf}
\end{tabular}
\caption{Generalized Legendre dual, $h(y)=\sup_{x\in \mathbb{S}^{d-1}} \rho(x)\langle x, y \rangle $, $\rho(x)=\inf_{y\in \mathbb{S}^{d-1}} h(y)/\langle x, y \rangle$. \label{fig:spherical_duality}}
\end{figure}

\section{Spherical Legendre Duality}

\begin{definition}[Radial Graph] Suppose $f:\mathbb{S}^2\to\mathbb{R}_+$ is a function defined on the sphere, then its radial graph is defined as 
\[
    \Gamma(f):=\{xf(x)|x\in\mathbb{S}^2\} \subset \mathbb{R}^3.
\] 
It is also denoted as $S_f$.
\end{definition}

\begin{definition}[Radial Representation] Suppose $S$ is a convex surface in $\mathbb{R}^3$, if there exists a function $\rho:\mathbb{S}^2\to\mathbb{R}_+$, such that $S=\Gamma(\rho)$, then we say $\rho$ is a radial representation of $S$.
\end{definition}
For example, a plane with normal $y$ and height $h$ has the radial representation
\[
    \pi:\mathbb{S}^2\to\mathbb{R}_+,\quad \pi(x) = \frac{h}{\langle y, x\rangle}.
\]
where $h$ is the distance from the origin to the plane, and called the \emph{height} of the plane. 

\begin{definition}[Generalized Legendre Dual] Suppose $\rho:\mathbb{S}^2\to\mathbb{R}_+$ is a positive spherical function, its generalized Legendre dual is a spherical function, $\rho^*:\mathbb{S}^2\to\mathbb{R}_+$, defined as
\begin{equation}
    \rho^*(y):= \sup_{x\in\mathbb{S}^2} \rho(x)\langle x, y \rangle.
    \label{eqn:spherical_legendre_dual}
\end{equation}
\end{definition}
The generalized Legendre dual of $S_\rho$ is the collection of its supporting planes. As shown in the left frame of figure \ref{fig:spherical_duality}, the geometric meaning of generalized Legendre dual can be interpreted as follows. Suppose $S_\rho$ is a convex surface in $\mathbb{R}^3$ with radial representation $\rho$. If we fix a direction $y\in\mathbb{S}^2$, there is the unique plane supporting $S_\rho$ with normal $y$, the height is $\rho^*(y)$.
Suppose the supporting plane $\rho^*(y)/\langle y, x \rangle$ touches $S_\rho$ at $\rho(x)x$, then 
\begin{equation}
    \rho^*(y)=\rho(x)\langle x,y \rangle.
    \label{eqn:Alexandrov_tangential_condition}
\end{equation}
For any other point $\tilde{x}\rho(\tilde{x})$ not touching the supporting plane, we have $\rho^*(y)>\rho(\tilde{x})\langle \tilde{x},y \rangle$.

Conversely, as shown in figure \ref{fig:spherical_duality} right frame, 
fix a point $x$ on $\mathbb{S}^2$, then
the ray starting from the origin and with the direction $x$ intersects all the supporting planes. The shortest distance from the origin to the intersection point is $\rho(x)$, namely
\begin{equation}
    \rho(x) = \inf_{y\in\mathbb{S}^2} \frac{\rho^*(y)}{\langle x, y \rangle}.
    \label{eqn:spherical_legendre_dual_inverse}
\end{equation}
Similarly, the equality holds if and only if the supporting plane $\rho^*(y)/\langle x, y\rangle$ touches the surface $S_\rho$ at $x\rho(x)$.

\begin{definition}[subnormal]Given a convex surface $S_\rho$ with radial representation $\rho:\mathbb{S}^2\to\mathbb{R}_+$, fix a point $x\in\mathbb{S}^2$, the subnormal at $x$ is defined as
\[
    \partial \rho(x):=\left\{y\in\mathbb{S}^2| \rho(x)\langle x,y \rangle \ge \rho(\xi)\langle \xi,y \rangle,\quad \forall \xi\in\mathbb{S}^2\right\}.
\]
Namely, the set of normals of supporting planes of $S_\rho$ at $x\rho(x)$.
\end{definition}

\begin{definition}[Gaussian Curvature Measure] Suppose a convex surface $S_\rho$ is with a radial representation $\rho:\mathbb{S}^2\to\mathbb{R}_+$. The subnormal map $\partial \rho$ is a set-valued map, 
\[
    \partial \rho:\mathbb{S}^2\to\mathbb{S}^2, \quad x\mapsto \partial \rho(x),
\]
The pull-back measure induced by $\partial \rho$ is called the Gaussian curvature measure, denoted as $\mu_\rho$. For any measurable set $\Omega\subset \mathbb{S}^2$,
\begin{equation}
    \mu_\rho(\Omega) = \text{Area}(\partial \rho(\Omega)).
\end{equation}
\end{definition}

\begin{figure}[t!]
    \centering
\begin{tabular}{c}
\includegraphics[height=0.45\textwidth]{figures/SphericalOMT/Alexandrov_solution.pdf}
\end{tabular}
\caption{Generalized Legendre dual, $h(y)=\max_{x\in \mathbb{S}^{d-1}} \rho(x)\langle x, y \rangle $, $\rho(x)=\min_{y\in \mathbb{S}^{d-1}} h(y)/\langle x, y \rangle$. \label{fig:Alexandrov_solution}}
\end{figure}

\subsection{Discrete Spherical Legendre Duality}
Suppose $\rho:\mathbb{S}^2\to\mathbb{S}^2$ is a discrete function $\rho(x)=\sum_{i=1}^k \rho_i\delta(x-x_i)$. The radial graph of $\rho$ is the convex hull of $\{\rho_ix_i\}$,
\begin{equation}
    S_\rho = \text{conv}(\{\rho_1x_1,\rho_2x_2,\dots,\rho_kx_k\}).
    \label{eqn:Alexandrov_convex_hull}
\end{equation}
The spherical Legendre dual $\rho^*:\mathbb{S}^2\to\mathbb{R}_+$ is a continuous function, (\ref{eqn:spherical_legendre_dual})
\begin{equation}
 \rho^*(y):= \max_{i=1}^k \rho_i\langle x_i, y \rangle, \quad\text{equivalently}~ 
 \frac{1}{\rho^*(y)} = \min_{i=1}^k \frac{1}{\rho_i}\frac{1}{\langle x_i, y \rangle}, 
    \label{eqn:spherical_legendre_dual_discrete}
\end{equation}
The spherical graph of $1/\rho*(y)$ is a convex polyhedron, which is the spherical envelope of planes. Each $x_i$ corresponds to a plane
\begin{equation}
    \pi_\rho^i(y)=\frac{1}{\rho_i\langle x_i,y\rangle}, 
    \label{eqn:Alexandrov_dual_plane}
\end{equation}
the spherical envelope of the planes is define as follows.

\begin{definition}[Spherical Envelope] Given functions defined on the sphere $f_1,\dots,f_k:\mathbb{S}^2\to \mathbb{R}_+$, the envelope of the functions $f_1,\dots, f_k$ is the graph of the function:
\[  
    f(y)=\min \left\{f_1(y),f_2(y),\dots, f_k(y)\right\}.
\]
namely
\[
    \text{env}\left(f_1,\dots,f_k\right) = \Gamma(f).
\]
\end{definition}
Then the spherical envelope of the planes $\pi_\rho^i$'s is given by
\begin{equation}
    S_{\rho^*}:=\text{env}\left(\pi_\rho^1,\pi_\rho^2,\dots,\pi_\rho^k\right) =
    \Gamma\left(\min\left\{\pi_\rho^1,\dots,\pi_\rho^k\right\}\right)=\Gamma\left(\frac{1}{\rho^*}\right).
\end{equation}    

The subnormal map induces a spherical cell decomposition. The subnormal of each face of $S_\rho$ is a single point, the subnormal of each vertex on the convex polyhedral $S_\rho$ is a spherical polygon, all these polyons form the cell decomposition.
\begin{definition}[Subnormal Cell Decomposition] Given a convex polyhedral surface $S_\rho$ with spherical representation $\rho=\sum_i^k \rho_i \delta(x-x_i)$, its subnormal map induces a spherical cell decomposition:
\begin{equation}
\mathbb{S}^2=\bigcup_{i=1}^k \partial \rho(x_i).
\label{eqn:subnormal_cell_decomposition}
\end{equation}
\end{definition}
\begin{definition}[Projection Cell Decomposition] Given a convex polyhedral surface $S_\rho$ with spherical representation $\rho=\sum_i^k \rho_i \delta(x-x_i)$, its generalized Legendre dual is $\rho^*$, the central projection to $S_{\rho^*}$ induces a cell decomposition
\begin{equation}
\mathbb{S}^2=\bigcup_{i=1}^k W_\rho(i), \quad W_\rho(i):=\left\{y\in\mathbb{S}^2| \pi_\rho^i(y)\le \pi_\rho^j(y),~\forall j~\right\}.
\label{eqn:central_projection_cell_decomposition}
\end{equation}
The area of $W_\rho(i)$ is denoted as $w_\rho(i)$.
\end{definition}

\begin{proposition}
Given a convex polyhedral surface $S_\rho$ with spherical representation $\rho=\sum_i^k \rho_i \delta(x-x_i)$, its generalized Legendre dual is $\rho^*$, the central projection to $S_{\rho^*}$. The subnormal cell decomposition (\ref{eqn:subnormal_cell_decomposition}) is identical to the cell decomposition induced by the central projection of $S_{\rho^*}$ (\ref{eqn:central_projection_cell_decomposition}). Therefore, this spherical cell decomposition can be denoted as $\mathcal{D}_\rho$.
\end{proposition}

\begin{proof}
Given a point $y\in\mathbb{S}^2$, according to (\ref{eqn:subnormal_cell_decomposition}) and (\ref{eqn:central_projection_cell_decomposition}), $\forall y\in \mathbb{S}^2$,
\[
y\in \partial \rho(x_i) \iff \rho_i\langle x_i, y \rangle \ge \rho_j\langle x_j, y \rangle~\forall~j~\iff \frac{1}{\rho_i\langle x_i,y\rangle}\le \frac{1}{\rho_j\langle x_j, y \rangle}~\forall~j\iff y\in W_i.
\]
\end{proof}

\begin{definition}[Spherical Weighted Delaunay Triangulation] Given a convex polyhedral surface $S_\rho$ with spherical representation $\rho=\sum_i^k \rho_i \delta(x-x_i)$, the induced spherical cell decomposition is $\mathcal{D}_\rho$. The weighted Delaunay triangulation $\mathcal{T}_\rho$ is the triangulation of $\{x_1,x_2,\dots,x_k\}$ dual to $\mathcal{D}_\rho$, given two cells $W_\rho(i), W_\rho(j)\in \mathcal{D}_\rho$, if their intersection is non-empty, then $x_i$ and $x_j$ are connected in $\mathcal{T}_\rho$:
\[
    W_\rho(i)\cap W_\rho(j) \neq \emptyset
     \iff x_i\sim x_j \in \mathcal{T}_\rho,\quad \forall i,j = 1,\dots, k.
\]
\end{definition}

\subsection{Computational Algorithm for Spherical Cell Decomposition}
\label{subsec:spherical_power_diagram}
The convex hull $S_\rho$, envelope $S_{\rho^*}$ and spherical cell decomposition $\mathcal{D}_\rho$ can be constructed as follows:

\begin{enumerate}
    \item $S_\rho$: According to definition (\ref{eqn:Alexandrov_convex_hull}), the convex polyhedron $S_\rho$ is obtained by the convex hull of points $\{\rho_1x_1,\dots, \rho_k x_k\}$. 
    \item $\mathcal{T}_\rho$: The weighted Delaunay triangulation $\mathcal{T}_\rho$ of $\{x_1,x_2,\dots,x_k\}$ has the same connectivity as $S_\rho$. 
    \item $\matcal{D}_\rho$: For each face $f_i$ on $S_\rho$, compute the normal $n_i$ to the face. The vertices of cell decomposition $\mathcal{D}_\rho$ are the normals. The connectivity of $\mathcal{D}_\rho$ is dual to that of $S_\rho$. Two faces $f_i$ and $f_j$ are adjacent on $S_\rho$, if and only if $n_i$ and $n_j$ are connected on $\mathcal{D}_\rho$. 
    \item $S_{\rho^*}$: The connectivity of $S_{\rho^*}$ is the same as that of $\mathcal{D}_\rho$. Each vertex $\rho_i x_i$ of $S_\rho$ corresponds to a face $\pi_\rho^i$ as in (\ref{eqn:Alexandrov_dual_plane}) of $S_{\rho^*}$. Each face in $S_\rho$ with vertices $\rho_i x_i, \rho_j x_j$ and $\rho_k x_k$ corresponds to a vertex in $S_{\rho^*}$, which is the intersection of $\pi_\rho^i,\pi_\rho^j$ and $\pi_\rho^k$. 
\end{enumerate}



    




\section{Spherical Diagram Theory}
%\subsection{Spherical Geometry}
\label{subsec:sgeo}
\subsection{Spherical Geodesics and Cosine Law}
A \emph{great circle} of $\mathbb{S}^{2}$ is a circle which intersects $\mathbb{S}^{2}$ with a plane passing through the center. \emph{Geodesics} are portion of some great circles on sphere. The \emph{geodesic distance} between two points $p,q$ on $\mathbb{S}^{2}$ is measured by the shortest arc length between them: $d(p,q) = \cos^{-1}\langle p,q\rangle$. Consider the points $A, B, C$ of a spherical triangle $\triangle$ on $\mathbb{S}^{2}$, as shown in Figure \ref{fig:sphere_triangle}. Let $a,b,c$ be the subtended angles at the center of $\mathbb{S}^{2}$. In fact, $a,b,c$ also measure the geodesic distances $d(B,C)$, $d(C,A)$, and $d(A,B)$.

Given a point $p_i$ on $\mathbb{S}^{2}$ and $0\leq r_{i}\leq \pi/2$. A \emph{geodesic circle} $c_i$ is defined by $c_i = \{p\in\mathbb{S}^{2}\mid d(p,p_i)=r_i\}$ where $p_i$ is the center and $r_i$ is the radius.
\begin{figure}[ht]
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.3\textwidth]{figures/SphericalOMT/sphere_triangle.png}\\
\end{tabular}
\end{center}
\caption{Triangle and circle on unit sphere}{\label{fig:sphere_triangle}}
\end{figure}

Let $A,B,C$ also denote the angles at $A,B,C$ respectively. The area of triangle on the sphere is
\begin{equation}
Area(\triangle) = A + B + C- \pi
\label{eqn:spherical_triangle_area}
\end{equation}
Let $a,b,c$ be the subtended angles at the center of $\mathbb{S}^{2}$. We have spherical cosine laws:
\begin{equation}
\cos c	=\cos a \cos b + \sin a \sin b \cos C
\label{eqn:spherical_cosine_law}
\end{equation}
and spherical sine law:
\begin{equation}
\frac{\sin a}{\sin A} = \frac{\sin b}{\sin B}= \frac{\sin c}{\sin C}.
\label{sphere_sin_law}
\end{equation}
For right triangle, suppose the angle at $C$ is $\pi/2$. Then the area is $Area(\triangle) = A + B - \pi/2$. Sides length and angles of right triangle have following relationship:
\begin{equation}
\cos c = \cos a \cos b
\label{eqn:spherical_cosine_law_right_triangle}
\end{equation}


\begin{algorithm2e}[ht!]
%\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{Genus $0$ closed surface $M$}
\KwOut{spherical area-preserving parameterization}

Compute conformal map from $M$ to unit sphere, $f:M\to\mathbb{S}^2$, obtain $\{x_i:=f(v_i)\}$;
Compute vertices' area of $M$ and normalize the total area to be $4\pi$, obtain $\mu$\;
Initialize the power radius $\rho = (\rho_1, \rho_2, \cdots, \rho_k) = (1,1,\dots,1)$\;
\While{true}{
\If {$ \|\nabla F\| < \varepsilon$} {
break\;
}

Compute power diagram $\mathcal{D}_\rho$ ;
Calculate gradient $\nabla {F}$ by Eqn.~\ref{eqn:spherical_OT_map_grad}\;
Calculate Hessian matrix $D^2F$ by Eqn.~\ref{eqn:alexandrov_hessian_element} and Eqn.\ref{eqn:diagonal_element};
Solve linear equation $ D^2 F h = \nabla{F}$\;

$\lambda \gets 1$\;

\While{true}{
    Compute the power diagram $\mathcal{D}_\rho$\;
    \If{$\forall W_\rho(i) \in \mathcal{D}_\rho$ not empty}{
    	break\;
    }
    $\lambda \gets \frac{1}{2} \lambda$\;
}
$\rho_i \gets \rho_i e^{\lambda h_i}$, $i=1,2,\dots,k$
}
Compute the mass center of each power cell $\forall \ W_\rho(i) \in \mathcal{D}_\rho$
\Return{the mapping from each vertex $v_i$ to the mass center of $W_i$ }\\
\caption{Spherical Area Preserving Parameterization}
\label{alg:SAPP}
\end{algorithm2e}




==> Minkowski.tex <==
\section{Minkowski Problem for Curvature Measures}

\begin{figure}[t!]
    \centering
\begin{tabular}{c}
\includegraphics[width=0.45\textwidth]{figures/normal_mapping.pdf}
\end{tabular}
\caption{Given a convex set $K\ni 0$, we can parameterize its boundary in plar coordinates using a map $\rho:\mathbb{S}^{d-1}\to \mathbb{R}^+$. Given a point $z\in \partial K$, the set $N_K(z)$ consists of all outer normals to $K$ at $z$. Such a set is a singleton when $K$ has a unique tangent plane (as for the point $z_2$), while it is multivalued at a corner point such as $z_1$. \label{fig:normal_mapping}}
\end{figure}

Let $K\subset \mathbb{R}^d$ be an open bounded convex domain containing the origin, and parameterize $\partial K$ in \emph{polar coordinates} as follows:
\[
    \partial K = \{ \rho(x)x: x\in \mathbb{S}^{d-1}, \rho: \mathbb{S}^{d-1}\to\mathbb{R}^+ \}.
\]
Then to any point $z\in \partial K$, we associate the \emph{normal mapping}
\begin{equation}
    N_K(z) := \left\{ y\in \mathbb{S}^{d-1}: K \subset \{ w: \langle y, w-z\rangle \le 0 \} \right\}.
    \label{eqn:normal_mapping}
\end{equation}
Geometrically, the normal mapping finds the normals of all supporting hyperplanes at $z$ (see Figure ~\ref{fig:normal_mapping}).
\begin{definition}[Gauss Map and Gaussian Measure]
The (multivalued) \emph{Gauss map} $G_K:\mathbb{S}^{d-1}\to\mathbb{S}^{d-1}$ is defined by $G_K(x):= N_K(\rho(x)x)$, and define the \emph{Gaussian curvature measure}
\[
    \mu_K(E):= \mathcal{H}^{d-1}(G_K(E))\quad \forall E\subset \mathbb{S}^{d-1}~\text{Borel}.
\]
where $\mathcal{H}^{d-1}$ denotes the $(d-1)$-dimensional Hausdorff measure on $\mathbb{S}^{d-1}$. 
\end{definition}
The famous Minkowski problem asks to reconstruct the shape from the Gaussian curvature measure.
\begin{problem}[Minkowski]
Given a Borel measure $\nu$ on $\mathbb{S}^{d-1}$, can one find an open bounded convex set $K\ni 0$ such that $\nu=\mu_K$?
\end{problem}

\begin{definition}[Spherical convex set and polar set]
Let $\omega\subset \mathbb{S}^{d-1}$, we say that $\omega$ is convex if the cone $\mathbb{R}^+\omega:=\{tx: t>0, x\in \omega\}$ is convex. We define the polar set to $\omega$ as $\omega^*:=\{ y\in \mathbb{S}^{d-1}:\langle x,y \rangle \le 0\quad \forall x\in \omega\}$.
\end{definition}
\begin{theorem}[Minkowski]
Let $\nu$ be a Borel measure on $\mathbb{S}^{d-1}$. Then
\[
    \nu = \mu_K~\text{for some}~K\quad\iff \left\{
    \begin{array}{clll}
    (a)& \nu(\mathbb{S}^{d-1})&=&\mathcal{H}^{d-1}(\mathbb{S}^{d-1})\\
    (b)& \nu(\mathbb{S}^{d-1}\setminus \omega) &>& \mathcal{H}^{d-1}(\omega^*)\\
    & \forall \omega\subsetneq \mathbb{S}^{d-1} &&~\text{compact and convex}
    \end{array}
    \right.
\]
In addition, if $K$ exists, then it is unique up to a dilation.
\label{thm:Minkowski}
\end{theorem}

Up to a change of coordinates, we can write $\partial K$ near $z_0$ as the graph of a convex function $u:\Omega\subset\mathbb{R}^d\to \mathbb{R}$. Suppose $u$ is $C^2$, then the Gaussian curvature of the graph of $u$ is 
\[
    \frac{det D^2 u}{(1+|\nabla u|^2)^{(d+2)/2}}.
\]
This shows that solving the Minkowski problem is equivalent to solve a Monge-Ampere type PDE. Suppose $\mu_K = fd\mathcal{H}^2$, where the density function $f$ is bounded, then by the regularity theory, the boundary $\partial K$ is $C^1$.


In the following, we prove the existence of the solution to the Minkowski problem. The uniqueness can be proven using Brunn-Minkowski inequality \cite{}.

\begin{figure}[t!]
    \centering
\begin{tabular}{c}
\includegraphics[height=0.45\textwidth]{figures/Alexandrov_Duality.pdf}
\end{tabular}
\caption{Generalized Legendre dual, $h(y)=\max_{x\in \mathbb{S}^{d-1}} \rho(x)\langle x, y \rangle $, $\rho(x)=\min_{y\in \mathbb{S}^{d-1}} h(y)/\langle x, y \rangle$. \label{fig:generalized_Legendre_dual}}
\end{figure}


\begin{definition}[Generalized Legendre Dual] Given a convex hypersurface in $\mathbb{R}^d$ with polar representation
\[
    S:= \{\rho(x)x: x\in \mathbb{S}^{d-1}, \rho:\mathbb{S}^{d-1}\to\mathbb{R}^+\},
\]
its generalized Legendre dual is
\[
    S^*:= \{ h(y)y: y\in \mathbb{S}^{d-1}, h:\mathbb{S}^{d-1}\to\mathbb{R}^+\}, 
\]
where
\begin{equation}
    h(y) := \sup_{x\in S} \rho(x) \langle x, y \rangle.
    \label{eqn:spherical_dual_1}    
\end{equation}
Symmetrically, $S=(S^*)^*$, and 
\begin{equation}
    \rho(x) = \inf_{y\in \mathbb{S}^{d-1}} \frac{h(y)}{\langle x,y\rangle}, 
    \label{eqn:spherical_dual_2}
\end{equation}
\end{definition}
Let $\varphi(x) := \log \rho(x)$, $\psi(y):=-\log h(y)$, the cost function $c(x,y):=-\log \langle x, y\rangle$, then $c$-transform is defined as
\[
    \varphi^c(y):= \inf_{x\in \mathbb{S}^{d-1}} c(x,y)-\varphi(x), \quad \psi^{\bar{c}}(x):= \inf_{y\in \mathbb{S}^{d-1}} c(x,y)-\psi(x).
\]
The uniqueness of  theorem~\ref{thm:Minkowski} can be proved by Brunn-Minkowski inequality. In the following, we prove the existence, the proof leads to a computational algorithm.
\begin{proof}
The Minkowski problem can be reformulated as an optimal transport problem: given a Borel measure $\nu$ on $\mathbb{S}^{d-1}$, find an optimal transport map $T:\mathbb{S}^{d-1}\to \mathbb{S}^{d-1}$, 
\[
    \inf_{T_\# \mathcal{H}^{d-1}=\nu} \int_{\mathbb{S}^{d-1}} -\log \langle x, T(x) \rangle d\mathcal{H}^{d-1}.
\]
This is equivalent to the Kantorovich dual problem:
\[
    \sup \left\{I(\varphi,\psi) , (\varphi,\psi)\in \mathcal{K} \right\}
\]
where the functional is defined as
\begin{equation}
    I(\varphi,\psi) = \int_{\mathbb{S}^{d-1}} \varphi(x) d\nu(x) +  \int_{\mathbb{S}^{d-1}} \psi(y) d\mathcal{H}^{d-1}(y)
    \label{eqn:functional}
\end{equation}
and the admissible function space is
\begin{equation}
    \mathcal{K} :=\left\{ (\varphi,\psi) \in (C(\mathbb{S}^{d-1}), C(\mathbb{S}^{d-1})): \varphi(x) +\psi(y) \le c(x,y) \right\}.
    \label{eqn:admissible_space}
\end{equation}
One can construct a sequence of function pairs $\{(\varphi_k,\psi_k)\}\subset \mathcal{K}$, where $\psi_k = \varphi_k^c$ and $\varphi_k=\psi_{k-1}^{\bar{c}}$. One can show that $I(\varphi_k,\psi_k)$ increases monotonously, and $\varphi_k,\psi_k$ are Lipstchitz continuous, with Lipschitz constant $\beta=\sup\{|Dc(x,y)|, x,y\in \mathbb{S}^{d-1}\}$. Fix one point $y_0\in \mathbb{S}^{d-1}$, let $\psi_k(y_0)=0$. By Lipschitz continuity, we get $\{\psi_k\}$ are uniformly bounded, hence $\{\varphi_k\}$ are also uniformly bounded. Up to a subsequence, we can assume $(\varphi_k,\psi_k)$ uniformly converge to $(\varphi^*,\psi^*)$, which are Lipschitz continuous and maximize the functional. This gives the existence. $\square$
\end{proof}


\section{Discrete Minkowski Problem}
In practice, the smooth Minkowski problem is generalized to the discrete case. In the following, we focus on the two dimensional spherical $\mathbb{S}^2$ situation. 

Suppose $K\subset\mathbb{R}^3$ is a compact convex set, its boundary $\partial K$ is a convex polyhedron. Without loss of generality, we assume $K$ contains the origin as an interior point, and $\partial K$ is triangulated. Assume the vertices of the polyhedron are $v_1,v_2,\cdots, v_n$, then $\partial K$ is the convex hull of its vertices $\partial K=\text{Conv}(\{v_i\}_{i=1}^n)$. The normal mapping Eqn.~(\ref{eqn:normal_mapping}) maps each vertex $v_i$ to a geodesic convex polygon $N_\rho(v_i)$ on the sphere, the spherical area the image of $N_\rho(v_i)$ is the Gaussian curvature measure of $v_i$, denoted as $K_i$. The Gaussian curvature $K_i$ can also be computed as the angle deficient, namely $2\pi$ minus the surrounding corner angles of $v_i$ on the polyhedron $\partial K$. 

Suppose the continuous radial function of $\partial K$ is $\rho(x)$, the height function of the supporting planes is $\eta(y)$. The vertices are given by $v_i = \rho_ix_i$, where $x_i$ is the radial direction of $v_i$. Then the graph $S_\rho$ equals to the polyhedron $\partial K$, $S_\rho$ is the convex hull of $\{\rho_ix_i\}_{i=1}^n$. Namely, $\rho(x)$ is fully determined on its values on $\{x_i\}_{i=1}^n$. The height function $\eta(y)=1/h(y)$ is the generalized Legendre dual of $\rho(x)$, 
\begin{equation}
   \eta(y) =\rho^*(x) = \min_{i=1}^k \left\{\frac{1}{\rho_i}\frac{1}{\langle x_i, y\rangle }\right\}.
   \label{eqn:envelope}
\end{equation}
On the right hand side, each $1/\rho_i\langle x_i, y \rangle$ is a plane in $\mathbb{R}^3$, denoted as $\pi_{x_i,\rho_i}$ with normal $x_i$ and height $1/\rho_i$. The radial graph $S^*$ of $\eta(y)$ is inner envelope of these planes, $S^*=\text{Env}\left(\{\pi_{x_i,\rho_i}\}_{i=1}^n\right)$. The center projection of $S^*$ induces a spherical cell decomposition, each face of $S^*$ is projected to a geodesic convex polygon $W_i(\rho)$,
\begin{equation}
    \mathbb{S}^2 = \bigcup W_{i}(\rho),\quad W_i(\rho):=\{y\in\mathbb{S}^2: \pi_{x_i,\rho_i}(y) \le \pi_{x_j,\rho_j}(y)\}.
\end{equation}
Note that $y\in W_i(\rho)$ is equivalent to $\rho_i\langle x_i,y \rangle \ge \rho_j\langle x_j, y\rangle$, $\forall j$, namely $y\in N_\rho(v_i)$. Therefore the cell $W_i$ equals to the normal mapping image of $v_i$, $W_i(\rho)=N_\rho(x_i)$, and the spherical area of $W_i(\rho)$ equals to the Gaussian curvature measure $K_i$ of $v_i$. The discrete Minkowski problem can be formulated as follows:
\begin{problem}[Discrete Minkowski]Given distinct points $\{x_1,x_2,\cdots, x_n\}$ on $\mathbb{S}^2$, such that no hemi-sphere contains all the points, given $\nu_1,\nu_2,\cdots, \nu_n>0$, $\sum_{i=1}^n \nu_i = 4\pi$, find positive numbers $\rho=(\rho_1,\rho_2,\cdots,\rho_n)$ such that the each vertex $v_i$ on the convex hull $S = \text{Conv}(\{\rho_ix_i\}_{i=1}^n)$ has the Gaussian curvature measure $\nu_i$, $i=1,2,\cdots,n$.
\end{problem}

Minkowski theorem can be generalized to the discrete situation directly. The radius function $\rho$ exists, and unique up to scaling. According to our proof, the computational process is reduced to optimizing the functional Eqn.~(\ref{eqn:functional}), which becomes to a simpler form in discrete case. In general, the Hausdorff measure $\mathcal{H}$ can be replaced by any Borel measure $\mu$ on the sphere with continuous density, and $\mu(W_i(\rho))$ is denoted as $w_i(\rho)$. Let $\varphi$ be $\log\rho$, $\psi$ be $\log\eta$, $\nu = \sum_{i=1}^n\nu_i \delta(y-x_i)$,
\begin{equation}
\begin{split}
    I(\varphi,\psi) &= \int_{\mathbb{S}^2} \varphi(x) d\nu(x) + \int_{\mathbb{S}^2} \psi(y) d\mu(y), \quad (\varphi,\psi)\in \mathcal{K}\\
    &= \sum_{i=1}^n\int_{W_i(\varphi)}\varphi^c d\mu(x) + \sum_{i=1}^n \varphi_i \nu_i, \quad \varphi_i = \varphi(x_i),\\
    &= \sum_{i=1}^n \int_{W_i(\varphi)} (c(x,x_i) - \varphi_i) d\mu(x) + \sum_{i=1}^n \varphi_i \nu_i\\
    &= \sum_{i=1}^n \int_{W_i(\varphi)} c(x,x_i) d\mu(x) + \sum_{i=1}^n \varphi_i (\nu_i-w_i(\varphi)).\\
\end{split}
\label{eqn:energy}
\end{equation}
Since $\nu$ is the sum of Dirac measures, $\varphi$ can be treated as a vector $(\varphi_1,\varphi_2,\dots,\varphi_n)$. 

\begin{lemma} The gradient of the energy 
\[
    I(\varphi_1,\cdots,\varphi_n) = \sum_{i=1}^n \int_{W_i(\varphi)} c(x,x_i) d\mu(x) + \sum_{i=1}^n \varphi_i (\nu_i-w_i(\varphi))
\]
is given by
\begin{equation}
    \nabla I(\varphi) = (\nu_1-w_1(\varphi),\nu_2-w_2(\varphi),\cdots, \nu_n - w_n(\varphi)), 
    \label{eqn:gradient}
\end{equation}
The Hessian is
\begin{equation}
    \frac{\partial^2 I(\varphi)}{\partial \varphi_i\partial \varphi_j} = -\frac{\partial w_i(\varphi)}{\partial \varphi_j} = -\frac{\partial w_j(\varphi)}{\partial \varphi_i}, \quad \frac{\partial^2 I(\varphi)}{\partial \varphi_i^2} = \sum_{i\neq j} \frac{\partial w_i(\varphi)}{\partial \varphi_j}
    \label{eqn:Hesian}
\end{equation}
Furthermore, the null space of the Hessian is $\text{Span}\{(1,1,\cdots,1)\}$, the energy is strictly concave on the complementary space of the null space.
\end{lemma}
\begin{proof} Suppose two cells $W_i(\varphi)$ and $W_j(\varphi)$ intersect with each other. Let $\varphi'=\varphi + \delta e_i$, where $e_i$ is the unit vector along the i-th coordinate axis. Then $W_i$ enlarges, $W_j$ shrinks. 
Suppose $x\in W_i(\varphi') \cap W_j(\varphi)$,
\[
\begin{split}
    x \in W_j(\varphi) \implies c(x,x_j) - \varphi_j &\le c(x,x_i) - \varphi_i\\
    x \in W_i(\varphi') \implies c(x,x_j) - \varphi_j & \ge c(x,x_i) - \varphi_i - \delta \\
\end{split}
\]
This shows 
\[
    0\le (c(x,x_i)-\varphi_i)-(c(x,x_j)-\varphi_j) \le \delta 
\]
Then we compute 
\[
\begin{split}
I(\varphi')-I(\varphi) &= -\delta w_i(\varphi) + \delta \nu_i + \sum_{j\neq i} \int_{W_j(\varphi)\cap W_i(\varphi')} [(c(x,x_i)-\varphi_i-\delta) - (c(x,x_j)-\varphi_j))]d\mu(x)\\
&=\delta(\nu_i-w_i(\varphi)) + \sum_{j\neq i} O(\delta)\mu(W_j(\varphi)\cap W_i(\varphi')).
\end{split}
\]
By the next lemma, we can see $\mu(W_j(\varphi)\cap W_i(\varphi'))$ is $O(\delta)$, therefore we get $I(\varphi+\delta e_i) - I(\varphi) = \delta(\nu_i - w_i(\varphi)) + O(\delta^2)$, hence we obtain the gradient formula $\partial I(\varphi)/\partial \varphi_i = \nu_i - w_i(\varphi)$. By the next lemma, $w_i(\varphi)$ is differentiable, so we obtain the formula for $\partial^2 I(\varphi)/\partial \varphi_i\partial \varphi_j$. Since
\[
    0 = \frac{\partial 4\pi }{\partial \varphi_i} = \sum_{j=1}^n \frac{\partial w_j(\varphi)}{\partial \varphi_i} = \sum_{j=1}^n \frac{\partial w_i(\varphi)}{\partial \varphi_j},
\]
we obtain $\partial w_i(\varphi)/\partial \varphi_i = \sum_{j\neq i} \partial w_i(\varphi)/\partial \varphi_j$. 

By geometric meaning, $\partial w_j/\partial \varphi_i <0$, hence the off diagonal elements of the Hessian matrix are non-negative. The Hessian matrix is diagonal dominant, hence its null space is one dimensional spaned by $(1,\dots,1)$. Otherwise, assume $v$ is in the null space, the $k$-th element of $v$ has the biggest absolute value, then the k-th element of $\text{Hess}v$ is non-zero, contradiction. The Hessian matrix is negative definite on the complementary space of the null space, this implies the strict concavity of the energy.
$\square$
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/spherical_power_diagram.pdf}
    \caption{Spherical weighted Delaunay triangulation $\mathcal{T}$ and power diagram $\mathcal{D}$ induced by the central projections of $S$ and $S^*$ and the geometric interpretation of the Hessian matrrix of the energy.
    \label{fig:spherical_power_diagram}}
\end{figure}
By construction, we have $S_\rho=\text{Conv}(\{\rho_ix_i\}_{i=1}^n)$ and $S_{\rho}^*=\text{Env}(\{\pi_{x_i,\rho_i}\})$. Each vertex $\rho_ix_i$ on $S$ is dual to a face $\pi_{x_i,\rho_i}$ of $S^*$, each face $[\rho_ix_i,\rho_jx_j,\rho_kx_k]$ is dual to a vertex $\pi_{x_i,\rho_i}\cap \pi_{x_j,\rho_j}\cap \pi_{x_k,\rho_k}$ on $S^*$. 
As shown in Fig.~(\ref{fig:spherical_power_diagram}), the central projection of $S_\rho$ onto $\mathbb{S}^2$ induces a geodesic spherical weighted Delaunay triangulation $\mathcal{T}$, the central projection of $S_\rho^*$ induces a geodesic spherical  power diagram $\mathcal{D}$. $\mathcal{T}$ and $\mathcal{D}$ are dual to each other. Suppose $[\rho_ix_i,\rho_jx_j,\rho_kx_k]$ is a face in $S$, its normal is $n_k$, its central projection $[x_i,x_j,x_k]$ is a face in $\mathcal{T}$. The edge $[x_i,x_j]$ in $\mathcal{T}$ is dual to $[n_l,n_k]$ in $\mathcal{D}$. 

\begin{lemma}Given the spherical weighted Delaunay triangulation $\mathcal{T}$ and the dual spherical power diagram $\mathcal{D}$, and $\mu$ is the uniform distribution, then
\begin{equation}
\frac{\partial w_j(\varphi)}{\partial \varphi_i} = \frac{\partial w_i(\varphi)}{\partial \varphi_j} = - \frac{\sin d_l + \sin d_k}{\tan d_i + \tan d_j}.
\end{equation}
\end{lemma}

\begin{proof} According to lemma 4 in \cite{}, 
\begin{equation}
\frac{\partial w_i(\varphi)}{\partial \varphi_j} = - \frac{1}{\rho_i\rho_j\sin(d_i+d_j)} \left( \frac{R_l^2\sin d_l}{\cos^2 d_l}+ \frac{R_k^2\sin d_k}{\cos^2 d_k} \right),
\label{eqn:hessian_element_1}
\end{equation}
where
\[
R_k = \rho_i\langle x_i, n_k \rangle = \rho_j\langle x_j, n_k \rangle = \rho_k\langle x_k, n_k \rangle.
\]
Since 
\[
\begin{split}
\rho_i \cos d(x_i,n_k) &= \rho_j \cos d(x_j,n_k) = R_k\\
\cos d(x_i,n_k) &= \cos d_i \cos d_k\\
\cos d(x_j,n_k) &=\cos d_j \cos d_k
\end{split}
\]
plug in to Eqn.~(\ref{eqn:hessian_element_1}), we obtain
\[
\frac{\partial w_i(\varphi)}{\partial \varphi_j} = - \frac{\cos d_i\cos d_j}{\sin(d_i+d_j)} \left( \sin d_l + \sin d_k\right) = -\frac{\sin d_l + \sin d_k}{\tan d_i + \tan d_j}.
\]
$\square$
\end{proof}



